SEER: Super-Optimization Explorer for HLS using E-graph Rewriting with MLIR

High-level synthesis (HLS) is a process that automatically translates a software program in a high-level language into a low-level hardware description. However, the hardware designs produced by HLS tools still suffer from a significant performance gap compared to manual implementations. This is because the input HLS programs must still be written using hardware design principles. Existing techniques either leave the program source unchanged or perform a fixed sequence of source transformation passes, potentially missing opportunities to find the optimal design. We propose a super-optimization approach for HLS that automatically rewrites an arbitrary software program into efficient HLS code that can be used to generate an optimized hardware design. We developed a toolflow named SEER, based on the e-graph data structure, to efficiently explore equivalent implementations of a program at scale. SEER provides an extensible framework, orchestrating existing software compiler passes and hardware synthesis optimizers. Our work is the first attempt to exploit e-graph rewriting for large software compiler frameworks, such as MLIR. Across a set of open-source benchmarks, we show that SEER achieves up to 38x the performance within 1.4x the area of the original program. Via an Intel-provided case study, SEER demonstrates the potential to outperform manually optimized designs produced by hardware experts.

==> imgs/message_calc_original_code.tex <==
\begin{minted}{c}
for (int j = 1; j < 4; j++) {
  for (int i = 0; i < 4; i++) {
    if (list[j][i] && message[i]) {
      sum++;
      message[0] = false;
      message[1] = false;
      message[2] = false;
      message[3] = false;
    }
    if (list[j][i])
      message[i] = true;
  }
}
\end{minted}

==> imgs/rewriting_rules_egg.tex <==
% \begin{table*}[]
% \centering
% \caption{SEER rewriting rules implemented directly in \egg. We present example datapath and gate level rewrites used, the total contains 106 rewrites~\cite{coward2022rover}. All datapath rewrites are signage and bitwidth dependent and conditionally applied to ensure correctness. We use $\overline{a}$ to denote the bitwise inverse of $a$. The \texttt{FMA} operator (fused-multiply add) captures logic synthesis optimizations.}
% \label{tab:rewriting_rules_egg}
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{m{8em} m{7em} m{10em} m{10em}}
% \toprule
% \makecell[c]{Class} & \makecell[c]{Rule Name} &  \makecell[c]{Left} & \makecell[c]{Right} \\
% \midrule
% Control Flow & Seq Assoc  & (\texttt{seq}\;a\;(\texttt{seq}\; b\; c)) & $(\texttt{seq}\; (\texttt{seq}\; a\; b)\; c)$ \\
% \cmidrule(lr){1-4}
%            & Left Shift Mul   & $(a\times b)\ll c$          & $(a\ll c) \times b$\\
%            & Mux Add          & $a \;?\; (b + c) : (d + e)$ & $(a \;?\; b : d) + (a \;?\; c : e)$\\
%            & Add Incr         & $(a\times b) + a$           & $(a+1)\times b$\\
% Datapath   & Shift to Mul     & $a\ll\text{const}$          & $a\times 2^\text{const}$\\
%            & Merge Left Shift & $(a\ll b)\ll c$             & $a\ll(b+c)$ \\
%            & Neg Not          & $-a$                        & $\overline{a} + 1$ \\
%            & FMA Merge        & $(a\times b)+c$             & \texttt{FMA}$(a, b, c)$ \\
% \cmidrule(lr){1-4}
%            & Xor And      & $(a\&b)\oplus(a\&c)$ & $a\&(b\oplus c)$  \\
%            & Or Not Same  & $(\overline{a}\|a)$ & $1$  \\
%            & And Not Same & $(\overline{a}\& a)$ & $0$  \\
% Gate Level & Xor Same     & $(a\oplus a)$ & $0$  \\
%            & Xor Zero     & $(a\oplus 0)$ & $a$  \\
%            & Xor One      & $(a\oplus 1)$ & $\overline{a}$  \\
%            & De Morgan    & $\overline{(a\& b)}$ & $\overline{a} \| \overline{b}$\\
        
% \bottomrule
% \end{tabular}
% % }
% \end{table*}
